A Scalable Querying Scheme for Memory-efficient Runtime Models with History

Runtime models provide a snapshot of a system at runtime at a desired level of abstraction. Via a causal connection to the modeled system and by employing model-driven engineering techniques, runtime models support schemes for (runtime) adaptation where data from previous snapshots facilitates more informed decisions. Nevertheless, although runtime models and model-based adaptation techniques have been the focus of extensive research, schemes that treat the evolution of the model over time as a first-class citizen have only lately received attention. Consequently, there is a lack of sophisticated technology for such runtime models with history. We present a querying scheme where the integration of temporal requirements with incremental model queries enables scalable querying for runtime models with history. Moreover, our scheme provides for a memory-efficient storage of such models. By integrating these two features into an adaptation loop, we enable efficient history-aware self-adaptation via runtime models, of which we present an implementation.

==> sections/implementation.tex <==
\section{Evaluation}\label{sec:evaluation}

\begingroup
\setlength{\textheight}{\the\dimexpr19.3cm+1\baselineskip}
% \setlength{\intextsep}{0pt}
\setlength{\textfloatsep}{.7\baselineskip plus 0.2\baselineskip minus 0.5\baselineskip}
\setlength{\belowcaptionskip}{0pt}
\setlength{\abovecaptionskip}{0pt}

\begin{figure}
	%\centering
	\includegraphics[width=\linewidth]{graphics/patterns}
	\caption{\label{fig:patterns}
		Illustrated Patterns of Running Example}
	\vspace{-3mm}
\end{figure}
\endgroup


\subsection{Implementation}
\label{subsec:implementation}

Our implementation is based on the Eclipse Modeling Framework (EMF), which is a widespread MDE technology for creating metamodels of architectures. For pattern matching, we employ the \emph{Story Diagram Interpreter} (SD) \cite{} and its indices-based optimization from \cite{Barkowsky2018}. SD uses \emph{local search} to start the search from a specific element of the graph and thus reduces the required effort for pattern matching~\cite{Hildebrandt14}.

For the removal of elements from the runtime model, we transparently replace the native EMF method with an optimized data structure and removal method via a \textsc{Java} agent which renders the removal more scalable. 

\subsection{Comparison to the tool \monpoly}

Monitoring temporal specifications by processing a trace of events which represent a system execution is at the epicenter of the field known as Runtime Monitoring \cite{DBLP:series/lncs/BartocciDDFMNS18}, although the application domains considered usually in RM differ from runtime models and self-adaptive scenarios. Nevertheless, we opted for a comparison with a state-of-the-art tool from the field, called \monpoly due to it being supported by a temporal logic which is as expressive as \MTGL, namely the Metric First-order Temporal Logic (MFOTL) \cite{Basin_2015_MonitoringMetricFirstOrderTemporalProperties} which employs first-order \emph{predicates}, i.e. relations, to capture system entities and their relationships. Also, the tool has ranked high in RM competitions and has been used in multiple comparisons with other tools. Although originally intended to detect violations of business policies expressed as a trace of timestamped relations, \monpoly can encode graphs and thus runtime models. We focus our comparison on three aspects:usability, performance and monitorability.

We interpret our SHS metamodel, log, and formulas based on a \monpoly setting in the following manner. For each vertex type in the metamodel we create a predicate whose arity is equal the number of vertex attributes plus a special attribute \emph{id}. The latter is needed to be able to refer to graph elements and capture the binding capabilities of \MTGL. Each edge in the metamodel is translated into a binary predicate. For instance, the nodes \emph{Probe} and \emph{MonitoringService} and their association is translated into the following predicates: \emph{probe(p\_id, status), mService(m\_id, patientID), probeToMService(p\_id, m\_id)}.

Because \monpoly reasons over specific temporal orderings of events, encoding a graph pattern as a property in \monpoly requires an explicit definition of the expected temporal ordering of the events corresponding to the creation of the pattern's elements. To emulate the pattern matching of \APPROACHNAME in the general case, we would therefore have to build an MFOTL formula that would consider all possible orderings of these events. In the case of $p_1$, which consists of 5 predicates (3 vertices and 2 edges, see \autoref{fig:patterns}) and thus requires 5 creation events, that would mean accounting for $5! = 120$ combinations. In our comparison, since the manner in which elements are added to our model always results in the same ordering of relevant events, we only account for that ordering in the formulation of the property.
Moreover, as the creation of any of the predicates may complete a match of the encoded pattern, we have to search for the remaining predicates using an unbounded past operator. The point that \monpoly's usability is sub-optimal when it comes to graph-based models and pattern matching becomes apparent.

\LS{mention that we also tried different formulations (including forward-looking search)}

Regarding the properties $\phi'_1$ and $\phi'_2$, we map the former in a straightforward manner to its MFOTL equivalent. This is not possible for  $\phi'_2$, as \monpoly restricts the use of negation in this case. It does so for reasons of monitorability, as \monpoly assumes an infinite domain of values, and the negation of a $p_3$ at a given timepoint when $p_3$ doesn't exist is satisfied by infinite values and thus non-monitorable. In the following, we compare to \monpoly only on results of $\phi'_1$.

\subsection{Experimental Setting}
\subsubsection{Simulator}
\subsubsection{Input traces}
%Real
The original dataset used for our experiments is a recording of 1050 patient trajectories that are admitted to the emergency ward of a hospital over the course of $1.5$ years~\cite{}. The original log contains several types of medical and logistical activities, among which, we are interested in the \textit{Release} activities for variants of discharge from the hospital, the activity indicating \textit{ER Sepsis Triage}, and the activity for \textit{IV Antibiotics}. The three types of activities together with their time stamps are kept in the log and remaining activity types are discarded from the log. We refer to this log as the \rl.
\begin{table}[b]\centering
 	\caption {Characteristics of the logs}
	\label{tab:logs}
 	\begin{tabular}{lr}\hline
 		& \multicolumn{1}{c}{\textbf{Fitted Probability Distribution}} \\
 		\cline{2-2} %\cmidrule{5-6}
 				
 \trace ($s$)& $Weibull(\num{3.7e+4},0.9)$  \\
 		
 	\sa ($s$) & $Weibull(\num{5.09e+3},0.59)$  \\
 		
 		\sr ($s$)&$Lognormal(13.15, 0.53)$\\ \hline
 	\end{tabular} 
\end{table}
\begin{figure}[t]
\begin{centering}
%\vspace{-7mm}
  \includegraphics[width=0.95\linewidth]{graphics/PHI-1Time.png}
  \caption{Time ($\phi_1$) }
  \label{fig:timefi1}
  \end{centering}
\end{figure}
To investigate our approach in presence of input logs with different density, that is the arrival rate of the patient activities, we derived three \textit{synthetic} logs from the \rl.  
%
%The \rl consists of three different activities, that is, \textit{ER Sepsis Triage}, \textit{IV Antibiotics} and \textit{Release}.
Each \textit{trace} in the log starts with a record of an \textit{ER Sepsis Triage} event. The inter arrival time between two subsequent \textit{ER Sepsis Triage} events defines the arrival rate of traces~(i.e.,~\trace). For each trace, starting with an \textit{ER Sepsis Triage} event, an \textit{IV Antibiotics} and \textit{Release} events might follow. The IAT between the \textit{ER Sepsis Triage} and \textit{IV Antibiotics} that is, \sa and the IAT between the \textit{ER Sepsis Triage} and \textit{Release} that is \sr are also captured from the \rl.
%
Using statistical probability distribution fitting, we  characterize the properties of the \rl. 
%
 
We select five probability distributions to test for fitting to \trace, \sa and \sr: exponential, Weibull, normal, lognormal, and gamma. The fitting of the probability distributions to the empirical datasets uses the Maximum Likelihood Estimation (MLE) method~\cite{}, which delivers good accuracy for the large data samples. Among the investigated distribution, we choose the one that maximises the loglikelihood value and minimises the AIC and BIC metrics\SG{SG explain these metrics in footnote?}. Table~\ref{tab:logs} shows the fitted probability distributions for the \rl.

%Synthetic logs
We extracted three \textit{synthetic} logs from \rl for the same period of time that is 1.5 years. We constructed three synthetic logs: x10, x100, and x1000 in which the density of the traces are respectively 10, 100, and 1000 times more than the \rl. 
%
We modified parameters of the \rl (cf. Table~\ref{tab:logs}) to obtain logs with extreme characteristic enabling us to study the impact
of extreme characteristics of input logs on the evaluated aspects of the approaches.
%
In addition, using multiple input logs with different characteristics for the experiments allows us to evaluate the robustness of the approaches and the obtained results. 

To construct the synthetic traces with 10, 100, and 1000 times more traces than the \rl, we generated x10, x100, and x1000 logs with \trace values that are $k=$ 10, 100, and 1000 times smaller than \trace values of the \rl. 
%
Using the probability distribution for \trace values, we construct set $S$ consisting of 1000 sample logs, each sample log includes 1050 \textit{ER Sepsis Triage} event that is the same number of traces as the \rl. 
%
 A normal distribution is extracted from $S$ to generate the synthetic logs. For this purpose, we randomly re-sampled $S$ using statistical bootstrapping~\cite{diciccio1996bootstrap} and formed a new set $S'$ of the mean values of each sampled log. The normal distribution $N(\frac{\mu'}{k}, \sigma'^2)$ generates \trace values for the envisioned synthetic logs.
 %
  $\mu'$ is mean value of set $S'$, value $k$ is set to 10, 100, and 1000 for generation of x10, x100, and x1000 logs respectively. This guarantees that the mean value of the synthesised \trace values is $k$ times smaller than the \rl.
 %
 Based on the 3-sigma rule, by defining $\sigma'=\frac{\mu'}{3k}$, the likelihood of negative \trace values in the synthesised logs reduces to $0.3\%$ (Cf.,~\cite{three-sigma-rule}). The negative values are trimmed form the logs in case of occurrence ($99.7\%$ confidence interval) 

%
To maintain comparability between the logs, the \sa and \sr values of the synthesized logs follow the same probability distribution as in the \rl.
%
\subsubsection{Approaches}
\begin{itemize}
    \item INTEMPO
    \item INTEMPO+
    \item MONPOLY
\end{itemize}
\subsubsection{Measurements}
\paragraph{Analysis Phase Of the MAPE}
\paragraph{FULL MAPE}

Resource consumption analysis
\begin{itemize}
    \item Memory
\end{itemize}
Performance analysis
\begin{itemize}
    \item Response time
\end{itemize}
Reliability analysis
\begin{itemize}
    \item Evaluate the guarantees that patients are attended to  within the shortest period ( before it is critical)(analysis correctness)
    \item Making correct decision (planning correctness)
\end{itemize}
\subsection{Results}
\begin{table}[b]\centering
 	\caption {Memory Consumption for $\phi_1$ (MB)}
	\label{tab:mem}
 	\begin{tabular}{l r r r}\hline
 
 	\multirow{2}{*}{\textbf{Approach}}&\multicolumn{3}{c}{\textbf{Input Log}}\\
 \cline{2-4}
 		& \textbf{Real} &\textbf{x10}&\textbf{x100}\\
 	
 		\hline%\cmidrule{5-6}
 				
 INTEMPO& 36&	139	&1150\\
 		
 	INTEMPO+ &  25&	26&	29
 \\
 		
 	MONPOLY&20&	31&	165\\ \hline
 	\end{tabular} 
\end{table}
\begin{figure}[t]
\begin{centering}
%\vspace{-7mm}
  \includegraphics[width=0.95\linewidth]{graphics/PHI-2Time.png}
  \caption{Time ($\phi_2$) }
  \label{fig:timefi2}
  \end{centering}
\end{figure}


\begin{figure}[t]
\begin{centering}
%\vspace{-7mm}
  \includegraphics[width=0.8\linewidth]{graphics/PHI-1TotalTime.png}
  \caption{Total Time ($\phi_1$)}
  \label{fig:totaltime}
  \end{centering}
\end{figure}

%\begin{figure}[t]
%\begin{centering}
%\vspace{-7mm}
 % \includegraphics[width=0.8\linewidth]{graphics/PHI-1Memory.png}
%  \caption{Memory Consumption ($\phi_1$)}
%  \label{fig:memory}
 % \end{centering}
%\end{figure}
%\newpage

\subsection{Threats to Validity}

Regarding internal validity, 

Regarding external validity, we first make remarks on our comparison to \monpoly. Comparison of a tool on an objective that is out of its scope should always be done with care; we strived to create a fair setting. Nonetheless, fundamental differences between \monpoly and \APPROACHNAME might still have an impact on our evaluation results: first \monpoly is not a pattern matching tool and our emulation of pattern matching might have space for improvement; secondly, \monpoly's semantics is point-based while \APPROACHNAME's is interval-based which affects results and performance in some cases; finally, for the property that \monpoly could not monitor, we remark that there might exist logically equivalent, monitorable formulas. Those formulas however would not correspond to the \MTGL formula in a straightforward manner. On a related note, in our simulation, i.e. a runtime model where there is only one invocation per patient, different modeling decisions might have improved performance. However, we deliberately restricted ourselves to the metamodel derived from real dataset and was adjusted to our SHS setting as we hold that such restrictions apply in the application domain in question. While this investigation can serve as an indication, to the scalability of our approach, quantitative claims on scalability require more extensive simulation scenarios.

%Threats to internal validity concerns how we performed the experiments and interpreted the results. We systematically investigated the scalability and memory consumption of the alternative solutions 
%by using a controlled simulation environment of a SHS. 
%Particularly, we are interested in the effects of incremental checking and data pruning on the performance scalability and memory consumption of a pattern matching mechanism. To solely focus on these effects, the two compared variants share identical monitoring, planning, and execution phases of the MAPE-K feedback loop and they use the same architectural runtime model. Moreover, the experiments draw from a medical guideline where instructions are deterministic and typically of the form \emph{condition-action}, and as such, enable replicating a simulation for the two variants and over
%multiple runs. This enables a fair comparison and the consideration of variations of the measured execution time for the pattern-matching. 

% external validity
%Threats to external validity may restrict the generalization of our evaluation results outside
%the scope of our experiments.
%We evaluated our approach on a simulated SHS using a synthesized event sequence. 
%SHS
%The systematic increase of the size of the sequence and, thus, the model size (number of patient sensors and pumps) allows for investigating the behavior of \APPROACHNAME under increasing complexity. While this investigation can serve as an indication, %to the scalability of our approach, 
%quantitative claims on scalability require extensive simulation scenarios that support a realistic setting for a large scale IoT system.
%Trace
%Synthetic data can limit the generality of experimental results. We nevertheless opted for it for a number of reasons: First, our focus was scalability whereas real sequences are typically used to assess fault-detection capabilities \cite{Dou_2017_AModelDrivenApproachtoTraceCheckingofPatternBasedTemporalProperties}. Secondly, because parameterizing data factors in a systematic way, such as the rate of generated events, helped us isolate and demonstrate key aspects of scalability that are relevant in IoT systems that produce voluminous streams of data. Finally, synthesized data allowed us to devise a scheme to monitor a real-world medical guideline which renders our approach relevant to IoT systems---particularly those related to healthcare.
